MemGuard: Defending against Black-Box Membership Inference Attacks via Adversarial Examples

In a membership inference attack, an attacker aims to infer whether a data sample is in a target classifier's training dataset or not. Specifically, given a black-box access to the target classifier, the attacker trains a binary classifier, which takes a data sample's confidence score vector predicted by the target classifier as an input and predicts the data sample to be a member or non-member of the target classifier's training dataset. Membership inference attacks pose severe privacy and security threats to the training dataset. Most existing defenses leverage differential privacy when training the target classifier or regularize the training process of the target classifier. These defenses suffer from two key limitations: 1) they do not have formal utility-loss guarantees of the confidence score vectors, and 2) they achieve suboptimal privacy-utility tradeoffs. In this work, we propose MemGuard, the first defense with formal utility-loss guarantees against black-box membership inference attacks. Instead of tampering the training process of the target classifier, MemGuard adds noise to each confidence score vector predicted by the target classifier. Our key observation is that attacker uses a classifier to predict member or non-member and classifier is vulnerable to adversarial examples. Based on the observation, we propose to add a carefully crafted noise vector to a confidence score vector to turn it into an adversarial example that misleads the attacker's classifier. Our experimental results on three datasets show that MemGuard can effectively defend against membership inference attacks and achieve better privacy-utility tradeoffs than existing defenses. Our work is the first one to show that adversarial examples can be used as defensive mechanisms to defend against membership inference attacks.

==> abstract_arxiv.tex <==
\begin{abstract}
In a membership inference attack, an attacker aims to infer whether a data sample is in a target classifier's training dataset or not. 
Specifically, given a black-box access to the target classifier, the attacker trains a binary classifier, which takes a data sample's confidence score vector predicted by the target classifier as an input and predicts the data sample to be a member or non-member of the target classifier's training dataset. 
Membership inference attacks pose severe privacy and security threats to the training dataset. Most existing defenses leverage differential privacy when training the target classifier or regularize the training process of the target classifier. These defenses suffer from two key limitations: 1) they do not have formal utility-loss guarantees of the confidence score vectors, and 2) they achieve suboptimal privacy-utility tradeoffs. 



In this work, we propose \emph{MemGuard}, the first defense with formal utility-loss guarantees against black-box membership inference attacks. Instead of tampering the training process of the target classifier, MemGuard adds noise to each confidence score vector predicted by the target classifier.  Our key observation is that attacker uses a classifier to predict member or non-member and classifier is vulnerable to \emph{adversarial examples}. Based on the observation, we propose to add a carefully crafted noise vector to a confidence score vector to turn it into an adversarial example that misleads the attacker's classifier. Specifically, MemGuard works in two phases. In Phase I, MemGuard finds a carefully crafted noise vector that can turn a confidence score vector into an adversarial example, which is likely to mislead the  attacker's classifier to make a random guessing at member or non-member. We find such carefully crafted noise vector via a new method that we design to incorporate the unique utility-loss constraints on the noise vector. 
In Phase II, MemGuard adds the noise vector to the confidence score vector with a certain probability, which is selected to satisfy a given utility-loss budget on the confidence score vector. Our experimental results on three datasets show that MemGuard can effectively defend against membership inference attacks and achieve better privacy-utility tradeoffs than existing defenses. Our work is the first one to show that adversarial examples can be used as defensive mechanisms to defend against membership inference attacks. 

\end{abstract}





==> macro.tex <==

\newcommand{\sample}{\mathbf{x}}
\newcommand{\sampleSpace}{\mathbf{X}}
\newcommand{\samplelabel}{\mathbf{y}}
\newcommand{\samplelabelSpace}{\mathbf{Y}}
\newcommand{\confscore}{\mathbf{s}}
\newcommand{\confscoreSpace}{\mathbf{S}}
\newcommand{\targetModel}{\mathcal{C}}
\newcommand{\attackModel}{\mathcal{A}}
\newcommand{\user}{u}
\newcommand{\noise}{\mathbf{n}}
\newcommand{\defenderAttackModel}{f}




==> system.tex <==
\section{Preliminaries}
\label{section:model}

In this section, we first define machine learning classification.
Then, we present the threat model.
In the end, we discuss our system model.

\subsection{Machine Learning}

In this work, we focus on machine learning classification, 
one of the most common ML applications~\cite{SSSS17,SZHBFB19,SBBFZ19}.
A machine learning classifier, denoted by $\targetModel$, is essentially a function
which maps a data sample $\sample$ to 
a vector of confidence scores $\confscore$.
Formally, we have:
\[
\targetModel: \sample \mapsto \confscore
\]
A confidence score vector $\confscore$ is also referred to as posterior probability:
Each entry of $\confscore$ indicates the probability of the corresponding data sample
being classified into a certain class or affiliated with a certain label.
The class with the highest probability is the final predicted class $\hat{\samplelabel}$ 
for the sample.
Meanwhile, we denote the real class label of the sample by $\samplelabel$.
For presentation purposes, we summarize the notations introduced here and later in this paper
in~\autoref{table:notations}.

\begin{table}[!t]
\centering
\caption{Notations, \YZ{we need add more notations}}
\label{table:notations}
\begin{tabular}{r|l} 
\toprule
Notation & Description\\
\midrule
$\sample$ & A data sample\\
$\confscore$ & A confidence score vector\\
$\samplelabel$ & Class label of a sample\\
$\targetModel$ & Target machine learning model\\
$\attackModel$ & Membership inference attack classifier\\
$\defenderAttackModel$ & Defender's membership inference classifier\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Threat Model}

Membership inference attack in the setting of machine learning
aims to determine whether a target data sample $\sample$
is in the training set of the target ML model $\targetModel$.
In this work, we concentrate on the black-box ML setting,
i.e., the adversary can only query the target model with the sample
and obtain the corresponding confidence score vector.
The adversary can only decide the membership of her target sample
based on the confidence score.
As pointed out by previous works~\cite{SSSS17,SBBFZ19}, 
this is the most difficult setting for the adversary.

A membership inference attack model, denoted by $\mathcal{A}$, 
can be formalized as the following map.
\[
\attackModel: \confscore \mapsto \{0, 1\}
\]
Here, $\confscore$ denotes the confidence score vector of the target data sample $\sample$, i.e., $\confscore=\targetModel(\sample)$, 
$1$ indicates $\sample$
is a member of the target model $\targetModel$'s training set and vice versa.
The attack model $\attackModel$ is also realized by an ML classifier.
An adversary can train $\attackModel$ in multiple ways depending on her knowledge
which is summarized as the following.

\begin{itemize}
    \item As previous works~\cite{SSSS17,SZHBFB19}, 
    we can assume that the adversary has some data samples coming from the same distribution as the training data of the target model.
    Then, she can establish a shadow model~\cite{SZHBFB19} or multiple shadow models~\cite{SSSS17} 
    to mimic the behavior of the target model.
    As the adversary controls the whole training process of her shadow models,
    she can derive the labeled data with respect to members and non-members,
    and utilize the data to train her attack model.
    One further assumption made by previous works is that the attacker knows the architecture of the target model.
    This can be realized by either using the same MLaaS API as the target model to establish shadow models~\cite{SSSS17}
    or performing model hyperparameter stealing attacks~\cite{WG18,OASF18}.
    %
    \item A different but stronger assumption in this direction is recently proposed by Nasr et al.~\cite{NSH18}.
    Specifically, they assume the attacker knows part of member and non-member data samples of target model.
    This indicates the attacker can directly train her attack model without building any shadow model.
    This attack is referred to as the sub-network attack.
    %
    \item The adversary can also know the underlying defense mechanism enforced by the target model.
    In this case, the adversary can establish her shadow model
    with the defense in place, and derive the adversarial training data for her attack model.
    We hypothesize that this attack, termed as the adaptive attack,
    results in a more robust membership inference against defense mechanisms.
\end{itemize}
Following these assumptions, we focus on 7 different membership inference attacks in this paper
such that our proposed defense mechanism can be evaluated comprehensively.







\subsection{System Model}
There are two parties in our system including user and defender.

\medskip
\myparatight{User}
We assume an user $\user$ has a training set and
denote it by $D_{\text{train}}^{\user}=\{\sampleSpace_{\text{train}},\samplelabelSpace_{\text{train}}\}$.
Here, $\sampleSpace_{\text{train}}=\{\sample_1,\cdots,\sample_{|\sampleSpace_{\text{train}}|}\}$ 
contains all the data samples and $\samplelabelSpace_{\text{train}}$ contains labels for each sample.
The user can use the training set to train a target model $\targetModel_{\user}$
and uses a testing set $D_{\text{test}}^{\user}=\{\sampleSpace_{\text{test}}, \samplelabelSpace_{\text{test}}\}$ 
to evaluate the performance of the model. 
% Given a query sample as input, the target model will output a confidence score vector and we use $\mathbf{s}$ to denote it, i.e., $\mathbf{s}=C_{u}(\mathbf{x})$. 
The goal of the user is to deploy $\targetModel_{\user}$ as a service
for others to query.
Specifically, the service will return a confidence score vector given a data sample. 
The user may suffer from recently proposed membership inference attack~\cite{SSSS17,SZHBFB19} 
by providing the original confidence score vector.
Instead, she relies on a defender to sanitize the confidence score vector.

\medskip
\myparatight{Defender} 
The defender is on the user side,
it can be an extra component of the user's deployed MLaaS,
or it can be an independent service provided by a trusted party.

The defender defends membership inference attack by adding a noise vector $\noise$ to the output of $\targetModel_{\user}$
given a data sample $\sample$.
This indicates the output of $\targetModel_{\user}$ on $\sample$ will be:
\[
\confscore'=\confscore+\noise
\]
% To defend against membership inference attack, the defender can add some random noise $\mathbf{n}$ to the output of $C_u$ given a query sample $\mathbf{x}$. 
% Specifically, the defender will output $\mathbf{s}^{\prime}=\mathbf{s}+\mathbf{n}$ and the noisy output will be returned as query result of the query sample $\mathbf{x}$. 
To calculate the noise,
the defender first builds a local membership inference classifier denoted by $\defenderAttackModel$
to assess the membership threat.
As the defender is on the user side, 
we assume it can access the user's training and testing sets as well as the target model.
This allows the defender to build the strongest membership inference classifier,
as it is trained on the ground truth data.
In detail, the defender first uses 
$\sampleSpace_{\text{train}}$ and $\sampleSpace_{\text{test}}$
to query $\targetModel_{\user}$,
and obtains the corresponding confidence scores 
denoted by $\confscoreSpace_{\text{train}}$ and $\confscoreSpace_{\text{test}}$, respectively.
All confidence score vectors in $\confscoreSpace_{\text{train}}$ are labeled as $1$, i.e., member samples, 
and $\confscoreSpace_{\text{test}}$ as $0$, non-member samples.
Then, $\defenderAttackModel$ is trained on this dataset.


